Beyond Joint Demonstrations: Personalized Expert Guidance for Efficient Multi-Agent Reinforcement Learning

Multi-Agent Reinforcement Learning (MARL) algorithms face the challenge of efficient exploration due to the exponential increase in the size of the joint state-action space. While demonstration-guided learning has proven beneficial in single-agent settings, its direct applicability to MARL is hindered by the practical difficulty of obtaining joint expert demonstrations. In this work, we introduce a novel concept of personalized expert demonstrations, tailored for each individual agent or, more broadly, each individual type of agent within a heterogeneous team. These demonstrations solely pertain to single-agent behaviors and how each agent can achieve personal goals without encompassing any cooperative elements, thus naively imitating them will not achieve cooperation due to potential conflicts. To this end, we propose an approach that selectively utilizes personalized expert demonstrations as guidance and allows agents to learn to cooperate, namely personalized expert-guided MARL (PegMARL). This algorithm utilizes two discriminators: the first provides incentives based on the alignment of individual agent behavior with demonstrations, and the second regulates incentives based on whether the behaviors lead to the desired outcome. We evaluate PegMARL using personalized demonstrations in both discrete and continuous environments. The experimental results demonstrate that PegMARL outperforms state-of-the-art MARL algorithms in solving coordinated tasks, achieving strong performance even when provided with suboptimal personalized demonstrations. We also showcase PegMARL's capability of leveraging joint demonstrations in the StarCraft scenario and converging effectively even with demonstrations from non-co-trained policies.

==> sections/algos-1.tex <==
\section{Expert Guided MARL Algorithm}



% \State Update the policy by maximizing the PPO-Clip objective:
% \begin{equation}
%     \theta_i^{k+1} = \arg \max _{\theta_i} \frac{1}{B^{k} T} \sum_{\tau \in \mathcal{B}^{k}} \sum_{t=0}^{T} \min \left(x, y\right)
% \end{equation}
% where
% $$x = \frac{\pi_{\theta_i}\left(a_{i}^t \mid s_{t}\right)}{\pi_{\theta_{i}^k}\left(a_{i}^t \mid s^{t}\right)} A^{\pi_{\theta_i^{k}}}\left(s^{t}, a_i^{t}\right)$$
% $$y = g\left(\epsilon, A^{\pi_{\theta_i^{k}}}\left(s_{t}, a_i^{t}\right)\right)$$


% %	\yuph{should the policy depends on $s_i^t$ or $o_i^t$?}


% \yuph{mark} 
% Utilizing expert guidance to deal with sparse rewards in a multi-agent RL setting is novel to our work. The multi-agent problem in~\eqref{defn:global-utility} becomes much more challenging when we are in sparse rewards settings. In single-agent settings, the authors in ~\citet{kang2018policy} propose learning from demonstrations (LfD) framework to use demonstrations to generate the occupancy measure for the expert policy and use that as a regularization term to the standard rewards objective. However, we cannot extend their approach in a straightforward manner to multi-agent settings because then it would require knowing the occupancy measures of the joint state-action pair for the expert demonstrations. 




%\review{[R1] The intuition behind using the shadow reward should be explained.}
In this section, we derive our first algorithm \textbf{E}xpert \textbf{G}uided \textbf{M}ulti-\textbf{A}gent \textbf{R}einforcement \textbf{L}earning (\textbf{EG-MARL}). According to \citet{zhang2021marl}, we can define shadow reward 
$r^{\pi}(s, a):=\frac{\partial F\left(\lambda^{\pi}\right)}{\partial \lambda(s, a)}$, which can be optimized by the agents to solve the aforementioned objective instead of reward $r(s,a)$. However, $r^{\pi}(s, a)$ depends on the global knowledge of all local utilities and thus is not suitable for the decentralized setting. Therefore, we  introduce the localized version of $r^{\pi}(s, a)$, the local shadow reward $r_{i}^\pi$ for each agent $i$:
\begin{equation}
    r_{i}^\pi :=\frac{\partial F_i\big(\lambda^{\pi_\theta}_{i}\big)}{\partial \lambda_{i}(s_{i}, a_{i})} 
    = r_{i}-\eta \log \left(\frac{2 \cdot {\lambda}_{i}^{\pi_\theta}\left(s_{i}, a_{i}\right)}{{\lambda}_{i}^{\pi_\theta}\left(s_{i}, a_{i}\right) + \lambda^{\pi_{E_i}}\left(s_{i}, a_{i}\right)}\right)  
    = r_{i} + \eta \bar{r}_i.
\label{eq:rrward}
\end{equation}
% \begin{equation}
% \begin{aligned}
%     r_{i}^\pi :&=\frac{\partial F_i\big(\lambda^{\pi_\theta}_{i}\big)}{\partial \lambda_{i}(s_{i}, a_{i})} \\
%     &= r_{i}-\eta \log \left(\frac{2 \cdot {\lambda}_{i}^{\pi_\theta}\left(s_{i}, a_{i}\right)}{{\lambda}_{i}^{\pi_\theta}\left(s_{i}, a_{i}\right) + \lambda^{\pi_{E_i}}\left(s_{i}, a_{i}\right)}\right)  \\
%     &= r_{i} + \eta \bar{r}_i.
% \end{aligned}
% \label{eq:rrward}
% \end{equation}
%
The first term $r_i$ is the original local reward, and the second term $\bar{r}_i$ can be viewed as an implicit personalized reward signal to augment the environmental exploration: 
\begin{itemize}[leftmargin=*]
	\item When ${\lambda}_{i}^{\pi_\theta}\left(s_{i}, a_{i}\right) < \lambda^{\pi_{E_i}}\left(s_{i}, a_{i}\right)$, indicating the probability of occupying the current state-action pair is smaller than the expert's, we have $\bar{r}_i > 0$, a positive incentive is added to the original reward to encourage the visitation frequency;
	\item When ${\lambda}_{i}^{\pi_\theta}\left(s_{i}, a_{i}\right) = \lambda^{\pi_{E_i}}\left(s_{i}, a_{i}\right)$, we have $\bar{r}_i = 0$, the probability matches the expert one's, so the original reward is not reshaped;
	\item When ${\lambda}_{i}^{\pi_\theta}\left(s_{i}, a_{i}\right) > \lambda^{\pi_{E_i}}\left(s_{i}, a_{i}\right)$, we have $\bar{r}_i < 0$, a negative incentive is added to the original reward to decrease the visitation frequency.
\end{itemize}
%


\begin{algorithm}[t!]
	\caption{\textbf{E}xpert \textbf{G}uided \textbf{M}ulti-\textbf{A}gent \textbf{R}einforcement \textbf{L}earning (EG-MARL)}
	\label{algo_EG-MARL}
	\raggedright
	\textbf{Input: } Agent number $N$; Initial parameters of policies and critics $\{\theta^0_i\}$ and $\{w^0_i\}$, where i = 1, 2, ..., N; Personalized expert trajectories $\{\mathcal{B}_{E_i} = \{(s_i^t, a_i^t)\}_{t=0}^H\}$ where i = 1, 2, ..., N; Batch size $\{B^k\}$; Episode length $\{H^k\}$; Weight parameters $\{\eta^k\}$.\\
	\raggedright
	\textbf{Output: } Learned policies $\{\pi_{\theta_i}\}$.
	\begin{algorithmic}[1]
		\For{agent $i=1, 2, ..., N$}
            \State Calculate empirical personalized expert state-action occupancy measures $\hat{\lambda}^{\pi_{E_i}}$ using equation \ref{eq:occ_mea}.
            % \begin{equation}
            %     \hat{\lambda}_{i}^{\pi_{E_i}}=\frac{1}{|\mathcal{B}_{E_i}|} \sum_{\tau \in \mathcal{B}_{E_i}} \sum_{t=0}^M \gamma^{t} \cdot \mathrm{e}\left(s_{E_i}^{t}, a_{E_i}^{t}\right)
            % \end{equation}
        \EndFor
        \For{iteration $k=0, 1, 2, ...$} 
		\State Perform $B^k$ multi-agent Monte Carlo rollouts to obtain trajectories $\tau = \{(s^t, a^t)\}_{t=0}^{H^k}$ with initial distribution $\xi$, policy $\pi_{\theta^k}$ collected as batch $\mathcal{B}^{k}$.
		\For{agent $i=1, 2, ..., N$}
        \State Compute empirical local occupancy measure $\hat{\lambda}_{i}^{\pi_{\theta}}$ using equation \ref{eq:occ_mea}.
		% \begin{equation}
		%     \hat{\lambda}_{i}=\frac{1}{B^k} \sum_{\tau \in \mathcal{B}^k} \sum_{t=0}^{H^k} \gamma^{t} \cdot \mathrm{e}\left(s_{i}^{t}, a_{i}^{t}\right)
		% \end{equation}
		\State Estimate the reshaped rewards $\hat{r}_{i}^{k}$ using equation \ref{eq:rrward}.
		\EndFor
		\State Compute averaged reward across all agents.
		\For{agent $i = 1, 2, ..., N$}
		\State Compute value estimates $V_i^t$ and advantage estimates ${A}_{i}^t$ based on the averaged reshaped rewards.
		\State Update $\theta_i$ by policy gradient:
		%\begin{equation}
		    $\mathbb{E}_{\mathcal{B}^k}\left[\nabla_{\theta_i} \pi_{\theta_i}(a_i | s) A_i(s, a_i)\right]$
		%\end{equation}
		
        \State Update $w_i$ to minimize the mean-squared loss: 
        % \begin{equation}
        %     \frac{1}{B^kT}\sum_{\tau \in \mathcal{B}^{k}} \sum_{t=0}^T\left[(V_{w_i}(s_t)-V_i^t)^2\right]
        % \end{equation}
        %\begin{equation}
           $ \mathbb{E}_{\mathcal{B}^k} \left[(V_{w_i}(s)-V_i)^2\right]$
       % \end{equation}
		\EndFor
		\For{agent $i = 1, 2, ..., N$}
		    \State Exchange information with neighbors $\mathcal{N}_i:=\{j: (i,j)\in \mathcal{E}\}$: 
		 %   \yuph{is the following equation okay? I want to take average over $w_i$ and all its neighbors}
		    %\begin{equation}
		        $w_i^{k+1} = \frac{1}{|\mathcal{N}_i|}\sum_{j\in\mathcal{N}_i} w_j^{k+1}$
		    %\end{equation}
		\EndFor
		\EndFor
        
	\end{algorithmic}
\end{algorithm}
The estimate of $r_i^\pi$ requires the calculation of personalized expert occupancy measures and local occupancy measures for each agent. In practice, we adopt Monte-Carlo rollouts to calculate them in a counting-based manner. Given a trajectory set $\mathcal{B}=\{(s^t, a^t)\}_{t=0}^H$, the empirical occupancy measure can be calculated as 
\begin{equation}
    \hat{\lambda}=\frac{1}{|\mathcal{B}|} \sum_{\tau \in \mathcal{B}} \sum_{t=0}^H \gamma^{t} \cdot \mathrm{e}\left(s^{t}, a^{t}\right),
    \label{eq:occ_mea}
\end{equation}
where $e(\cdot)$ is an indicator function. The personalized expert demonstrations are single-agent interactions with the environment, so we can use the above equation to calculate the associated occupancy measures directly. To calculate the local occupancy measure using multi-agent trajectories, we get the local state component from the global state, and replace $\mathrm{e}\left(s^{t}, a^{t}\right)$ with $\mathrm{e}\left(s_i^{t}, a_i^{t}\right)$ instead.

To solve the problem in a model-free manner, we proposed a decentralized actor-critic-based algorithm summarized in Algorithm~\ref{algo_EG-MARL}. It is compatible with any policy gradient methods, \eg, TRPO \citep{schulman2015trust} and PPO \citep{schulman2017proximal}. We adopted PPO-based actor updates in our implementation. 

\begin{algorithm}[t!]
	\caption{\textbf{G}eneralized \textbf{E}xpert \textbf{G}uided \textbf{M}ulti-\textbf{A}gent \textbf{R}einforcement \textbf{L}earning (GEG-MARL)}
	\label{algo_GEG-MARL}
	\raggedright
	\textbf{Input: } Agent number $N$; Initial parameters of policies, discriminators, and critics $\{\theta^0_i\}$, $\{\phi^0_i\}$, $\{w^0_i\}$, where i = 1, 2, ..., N; Personalized expert trajectories $\{\mathcal{B}_{E_i} = \{(s_i^t, a_i^t)\}_{t=0}^H\}$ where i = 1, 2, ..., N; Batch size $\{B^k\}$; Episode length $\{H^k\}$; Weight parameters $\{\eta^k\}$.\\
	\raggedright
	\textbf{Output: } Learned policies $\{\pi_{\theta_i}\}$.
	\begin{algorithmic}[1]
		% \State {\bfseries Input:} Agent number $N$; Initial parameters of policies and critics $\{\theta^0_i\}$ and $\{w^0_i\}$, where i = 1, 2, ..., N; Batch size $\{B^k\}$; Episode length $\{H^k\}$; Weight parameters $\{w^k\}$
		% \State {\bfseries Output:} Learned policies $\{\pi_{\theta_i}\}$ 
		\For{iteration $k=0, 1, 2, ...$} 
		\State Perform $B^k$ multi-agent Monte Carlo rollouts to obtain trajectories $\tau = \{(s^t, a^t)\}_{t=0}^{H^k}$ with initial distribution $\xi$, policy $\pi_{\theta^k}$ collected as batch $\mathcal{B}^{k}$.
		\For{agent $i=1, 2, ..., N$}
		\State Update $\phi_i$ to increase the objective
		\begin{equation}
		    \mathbb{E}_{\mathcal{B}^k}\left[\log D_{\phi_i}(s_i, a_i)\right]+\mathbb{E}_{\mathcal{B}_{E_i}}\left[\log (1-D_{\phi_i}(s_i, a_i))\right]
		\end{equation}
		\State Estimate the reshaped reward as
       % \begin{equation}
            $\hat{r}_{i}^{k}=r_i - \eta^k \log D_{\phi_i}(s_i, a_i)$
       % \end{equation}
		\EndFor
  \State Step 10-18 in Algorithm \ref{algo_EG-MARL}.
% 		\State Compute averaged reward across all agents.
% 		\For{agent $i = 1, 2, ..., N$}
% 		\State Compute value estimates $V_i^t$ and advantage estimates ${A}_{i}^t$ based on the averaged reshaped rewards.
% % 		\State Compute rewards-to-go $\hat{R}_{i}^t$ using the reshaped reward.
% % 		\State Compute averaged rewards-to-go $\bar{R}^t = \frac{1}{N} \sum\hat{R}_{i}^t$.
% % 		\State Compute advantage estimates, $\hat{A}_{i}^t$ based on the current value function $V_{w^k_i}$ and the averaged rewards-to-go $\bar{R}^t$.
% 		\State Update $\theta_i$ by policy gradient:
% 		\begin{equation}
% 		    \mathbb{E}_{\mathcal{B}_k}\left[\nabla_{\theta_i} \pi_{\theta_i}(a_i | s) A_i(s, a_i)\right]
% 		\end{equation}
		
%         \State Update $w_i$ to minimize the mean-squared loss: 
%         % \begin{equation}
%         %     \frac{1}{B^kT}\sum_{\tau \in \mathcal{B}^{k}} \sum_{t=0}^T\left[(V_{w_i}(s_t)-V_i^t)^2\right]
%         % \end{equation}
%         \begin{equation}
%             \mathbb{E}_{\mathcal{B}_k} \left[(V_{w_i}(s)-V_i)^2\right]
%         \end{equation}
% 		\EndFor
% 		\For{agent $i = 1, 2, ..., N$}
% 		    \State Exchange information with neighbors:
% 		 %   \yuph{is the following equation okay? I want to take average over $w_i$ and all its neighbors}
% 		    \begin{equation}
% 		        w_i^{k+1} = \frac{1}{|\mathcal{N}_i|}\sum_{j\in\mathcal{N}_i} w_j^{k+1}
% 		    \end{equation}
% 		\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}
% The occupancy measure is calculated through Monte-Carlo rollouts, and the implicit reward is further calculated. This process is summarized in Algorithm \ref{algo_2}. 
%\PT{Need to describe the algorithm a bit.. specifically what ``exchange information'' means}



% where we use PPO-based actor updates




% \begin{algorithm}[t!]
% 	\caption{\textbf{E}xpert \textbf{G}uided \textbf{M}ulti-\textbf{A}gent \textbf{R}einforcement \textbf{L}earning (EG-MARL)}
% 	\label{algo_EG-MARL}
% 	\raggedright
% 	\textbf{Input: } Agent number $N$; Initial parameters of policies and critics $\{\theta^0_i\}$ and $\{w^0_i\}$, where i = 1, 2, ..., N; Expert trajectories $\{\mathcal{B}_{E_i} = \{(s_i^t, a_i^t)\}_{t=0}^M\}$ where i = 1, 2, ..., N; Batch size $\{B^k\}$; Episode length $\{H^k\}$; Weight parameters $\{\eta^k\}$.\\
% 	\raggedright
% 	\textbf{Output: } Learned policies $\{\pi_{\theta_i}\}$.
% 	\begin{algorithmic}[1]
% 		\For{iteration $k=0, 1, 2, ...$} 
% 		\State Perform $B^k$ Monte Carlo rollouts to obtain trajectories $\tau = \{(s^t, a^t)\}_{t=0}^{H^k}$ with initial distribution $\xi$, policy $\pi_{\theta^k}$ collected as batch $\mathcal{B}^{k}$.
% 		\State Estimate implicit rewards $\{\bar{r}_i^k\}$ using Algorithm \ref{algo_2}.
% 		\For{agent $i=1, 2, ..., N$}
% 		\State Estimate the reshaped reward as
%         \begin{equation}
%             \hat{r}_{i}^{k}=r_i + \eta^k \cdot \bar{r}_i^k
%         \end{equation}
% 		\EndFor
% 		\State Compute averaged reward across all agents.
% 		\For{agent $i = 1, 2, ..., N$}
% 		\State Compute value estimates $V_i^t$ and advantage estimates ${A}_{i}^t$ based on the averaged reshaped rewards.
% 		\State Update $\theta_i$ by policy gradient:
% 		\begin{equation}
% 		    \mathbb{E}_{\mathcal{B}_k}\left[\nabla_{\theta_i} \pi_{\theta_i}(a_i | s) A_i(s, a_i)\right]
% 		\end{equation}
		
%         \State Update $w_i$ to minimize the mean-squared loss: 
%         % \begin{equation}
%         %     \frac{1}{B^kT}\sum_{\tau \in \mathcal{B}^{k}} \sum_{t=0}^T\left[(V_{w_i}(s_t)-V_i^t)^2\right]
%         % \end{equation}
%         \begin{equation}
%             \mathbb{E}_{\mathcal{B}_k} \left[(V_{w_i}(s)-V_i)^2\right]
%         \end{equation}
% 		\EndFor
% 		\For{agent $i = 1, 2, ..., N$}
% 		    \State Exchange information with neighbors $\mathcal{N}_i:=\{j: (i,j)\in \mathcal{E}\}$: 
% 		 %   \yuph{is the following equation okay? I want to take average over $w_i$ and all its neighbors}
% 		    \begin{equation}
% 		        w_i^{k+1} = \frac{1}{|\mathcal{N}_i|}\sum_{j\in\mathcal{N}_i} w_j^{k+1}
% 		    \end{equation}
% 		\EndFor
% 		\EndFor
% 	\end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[t]
% 	\caption{Implicit Reward Estimation through Monte-Carlo Rollout}\label{algo_2}
% 	\raggedright
% 	\textbf{Input: } Agent number $N$; Current parameters of policies $\{\theta_i\}$, where i = 1, 2, ..., N; Batch size $B$; Episode length $H$; Prior state-action occupancy measure $\left\{\lambda_{i}^{\pi_{E_i}}\left(s_{i}, a_{i}\right)\right\}$ for each agent estimated from demonstration trajectories.\\
% 	\raggedright
% 	\textbf{Output: } Estimated implicit rewards $\{\bar{r}_i\}.$
% 	\begin{algorithmic}[1]
% 		\State Perform $B$ Monte Carlo rollouts to obtain trajectories $\tau = \{(s^t, a^t)\}_{t=0}^H$ with initial distribution $\xi$, policy $\pi_{\theta}$ collected as batch $\mathcal{B}$.
% 		\For{agent $i=1, 2, ..., N$}
% 		\State Compute empirical local occupancy measure
% 		\begin{equation}
% 		    \hat{\lambda}_{i}=\frac{1}{B} \sum_{\tau \in \mathcal{B}} \sum_{t=0}^{H} \gamma^{t} \cdot \mathrm{e}\left(s_{i}^{t}, a_{i}^{t}\right)
% 		\end{equation}
% 		\State Estimate implicit reward 
% 		\begin{equation}
% 		    \bar{r}_i= -\log \left(\frac{2 \cdot \hat{\lambda}_{i}^{\pi_\theta}\left(s_{i}, a_{i}\right)}{\hat{\lambda}_{i}^{\pi_\theta}\left(s_{i}, a_{i}\right) + \lambda_{i}^{\pi_{E_i}}\left(s_{i}, a_{i}\right)}\right)
% 		\end{equation}
% 		\EndFor
% 	\end{algorithmic}
% \end{algorithm}


==> sections/algos-2.tex <==
\section{Generalized Expert Guided MARL Algorithm}

%\review{[R1] The second concern is that the presentation needs to be improved significantly: for example, the derivation of GE-A is confusing. The authors first introduce the bound with additional entropy penalties, and then come up with the minimax formulation resembling Kang et al, and then they derive another objective that apparently changes the expert demonstrations (discriminator). This appears to be too heuristic and not well justified.}

%\review{[R1]  Is the bottleneck of estimating occupancy measures mainly caused by the combinatorial explosion of the multi-agent setting, or simply by a large-state space for a single agent?}

We note that the major bottleneck with Algorithm \ref{algo_EG-MARL} is associated with the occupancy measure estimation. This step becomes quite expensive when the state space is large, making the algorithm ineffective, and even impractical when the state and action space are continuous. We deal with this issue by utilizing the idea from~\citet{ho2016generative}, which replaces the JS divergence to the expert's demonstration with
%
%\begin{theorem}[From \citet{kang2018policy}]
%Let $h(u) = \log(\frac{1}{1+e^{-u}})$, $\bar{h}(u) = \log(\frac{e^{-u}}{1+e^{-u}})$ and $U(s, a): \mathcal{S} \times \mathcal{A} \longrightarrow \mathbb{R}$ be an arbitrary function. Then we have
%
\begin{equation}
\label{JS_divergence}
D_{JS}(\lambda_\pi, \lambda_E) \approx
 \sup_D(\mathbb{E}_{\lambda_\pi}[\log(D(s, a))] + \mathbb{E}_{\lambda_E}[\log(1-D(s,a))]),
\end{equation}

% \begin{align}\label{JS_divergence}
% 	D_{JS}&(\lambda_\pi, \lambda_E) \approx
%  \\&\sup_D(\mathbb{E}_{\lambda_\pi}[\log(D(s, a))] + \mathbb{E}_{\lambda_E}[\log(1-D(s,a))]), \nonumber
% \end{align}
%
where $D(s, a): \mathcal{S} \times \mathcal{A} \longrightarrow \mathbb{R}$  is discriminative classifier. 
%\end{theorem}
%
% To learn more about the derivative details, the reader is kindly referred to the supplemental of \citet{kang2018policy}. 
 Next, we utilize the lower bound mentioned in \eqref{JS_divergence} into 
 %, 
 %uilding on this result for the single agent setting from \citet{kang2018policy}, the local occupancy measure objective $\mathcal{L}_i$ in Equation (\ref{defn:global-utility-2}) can be written as:
% \begin{equation}
% \begin{aligned}
%     \mathcal{L}_i \triangleq \sup_{D\in(0,1)} \mathbb{E}_{\pi_{\theta_i}}&[\log(D(s_{i}, a_{i}))] + \\ &\mathbb{E}_{\pi_{E_i}}[\log(1 - D(s_{i}, a_{i}))],
% \end{aligned}
% \end{equation}
% % {\mathcal{S}_i \times \mathcal{A}_i}
% where $D(s_i, a_i) = \frac{1}{1+e^{-U(s_i, a_i)}}: \mathcal{S}_i\times\mathcal{A}_i\longrightarrow (0, 1)$ is an arbitrary mapping function followed by a sigmoid activation function for scaling. The supremum ranging over $D(s_i, a_i)$ is equivalent to the optimal binary classification loss of distinguishing the current local policy $\pi_{\theta_i}$ and the corresponding personalized expert policy $\pi_{E_i}$ w.r.t. the local state-action pairs sampled from $\lambda^{\pi_{\theta}}_{i}$ and the state-action pairs sampled from $\lambda^{\pi_{E_i}}$.
% %
% %
% Therefore, the overall objective of Equation 
\eqref{defn:global-utility-2}, and rewrite the objective as 
%
%\begin{equation}
\begin{align}\label{modified_problem}
    \min_\theta \sup_{D\in(0,1)}&(-R(\pi_\theta,D)),
\end{align}
%\end{equation}
%
where objective $R(\pi_\theta,D)$ is given by
%
\small
\begin{equation}\label{objective}
    R(\pi_\theta,D) = \frac{1}{N}\sum_{i=1}^N \big[\ip{\lambda^{\pi_{\theta}}_{i},r_i} + \beta H_i(\pi_{\theta_i})  -\eta\mathbb{E}_{\pi_{\theta_i}}[\log(D(s_i, a_i))] 
  -  \mathbb{E}_{\pi_{E_i}}[\log(1 - D(s_i, a_i))] \big].
\end{equation}
\normalsize
% \begin{align}\label{objective}
%     R(\pi_\theta,D) = \frac{1}{N}\sum_{i=1}^N \big[&\ip{\lambda^{\pi_{\theta}}_{i},r_i} + \beta H_i(\pi_{\theta_i})  
%     \\
%     &\hspace{-2cm}-\eta\mathbb{E}_{\pi_{\theta_i}}[\log(D(s_i, a_i))] 
%   -  \mathbb{E}_{\pi_{E_i}}[\log(1 - D(s_i, a_i))] \big].\nonumber
% \end{align}
% {\mathcal{S} \times \mathcal{A}}
In \eqref{objective},  $H_i\left(\pi_{\theta_i}\right)$ is for entropic regularization to avoid overfitting \citep{ziebart2008maximum, ziebart2010modeling}, and $\beta$ is a hyperparameter that weighs the regularization.
%
%
We note that the problem in \eqref{modified_problem} is a minimax problem similar to the target in Generative Adversarial Networks (GANs)~\citep{goodfellow2014generative}. GANs aim to learn a generative model to produce samples that cannot be distinguished from the true distribution even with a well-trained discriminative model. In our case, the true distributions are the personalized expert policies $\pi_{E_i}(a_i|s_i)$, or equivalently the expert occupancy measures $\lambda^{\pi_{E_i}}$. Our approach is different from imitation learning in the sense that we only use personalized demonstrations as guidance rather than fully mimicking the expert demonstration. Suppose $D_i$ is parameterized by $\phi_i$. By labeling expert individual state-action pairs as true (“1”) and policy local state-action pairs as false (“0”), we get the following objective:
\small
\begin{equation}
    \min_\theta \max_\phi \mathcal{L} = \frac{1}{N}\sum_{i=1}^N \big[ -\ip{\lambda^{\pi_{\theta}}_{i},r_i} - \beta H_i(\pi_{\theta_i})   +\eta(\mathbb{E}_{\pi_{\theta_i}}[\log(D_{\phi_i}(s_i, a_i))] +  \mathbb{E}_{\pi_{E_i}}[\log(1 - D_{\phi_i}(s_i, a_i))]) \big].
\end{equation}
\normalsize
% \begin{equation}
% \begin{aligned}
%     \min_\theta & \max_\phi \mathcal{L} = \frac{1}{N}\sum_{i=1}^N \big[ -\ip{\lambda^{\pi_{\theta}}_{i},r_i} - \beta H_i(\pi_{\theta_i})  \\
%     & +\eta(\mathbb{E}_{\pi_{\theta_i}}[\log(D_{\phi_i}(s_i, a_i))] +  \mathbb{E}_{\pi_{E_i}}[\log(1 - D_{\phi_i}(s_i, a_i))]) \big].
% \end{aligned}
% \end{equation}
%
% \yuph{text copied from \citet{kang2018policy}, modified according to our context, but the sentences and logic are still quite similar to their. Further rewriting would be good.}
%
Algorithm \ref{algo_GEG-MARL} presents the details of how we solve this optimization problem. We refer this algorithm as Generalized EG-MARL (GEG-MARL) to reflect the generalization ability provided by training a discriminator, rather than empirical estimation of local occupancy measures as in EG-MARL. As we show in the next section, GEG-MARL generalizes better to increasing number of agents as well as to continuous state-action spaces. 


% \begin{figure}[h!]
% 	\centering
% 	\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
% 	\caption{Sample figure caption.}
% \end{figure}



==> sections/exp_backup.tex <==


\section{Experiments}

In this section, we investigate the performance of EG-MARL and GEG-MARL empirically. We focus on the following questions: (1) how do EG-MARL and GEG-MARL that leverage personalized demonstrations compare to state-of-the-art MARL techniques? (2) how does the sub-optimality of the personalized expert demonstrations affect the performance of EG-MARL and GEG-MARL? and (3) how do EG-MARL and GEG-MARL scale with an increasing number of agents and in case of continuous state-action spaces?
%  for imitation learning and for learning a policy without demonstrations
% (2) how well does the Monte-Carlo implicit reward estimate the local occupancy measure in terms of the eventual EG-MARL policy; 

We consider three environments, two discrete and one continuous, for our evaluation. The two discrete environments require different levels of collaboration. 
We start by describing the experiments conducted on the discrete gridworld environments and then present results for the continuous case.

% \review{[R2] Does an expert's demonstration have to be consistent with the learning goal in eq. 6? How could the quality of an expert's demonstration affect final policies? The optimal policies shown in fig. 3 do not seem to be truly optimal, since agents will still collide with each other.}

% \review{[R2] Lastly, does individual-level demonstration work when optimal joint action requires two agents perform specific individual actions at the same time?}

% \review{[R3] From a different perspective, could this method be used when joint demonstrations are available? How would it compare with prior multi-agent LfD methods?}

% \subsection{Discrete Gridworld Environments}
\subsection{Comparison with the Existing Methods}
We use two gridworld environments with discrete state and action space: the lava scenario (Figure \ref{fig:lava}) and the door scenario (Figure \ref{fig:appledoor}). The agents in the lava scenario are homogeneous in that they have the same objective: navigate to their corresponding goal location. The door scenario is heterogeneous: the assistant agent (green) needs to open the door while the other agent (red) needs to reach the goal. 



\begin{figure}
\begin{minipage}[c]{0.55\linewidth}
  \centering
  \setlength\tabcolsep{1.5pt}
  \fontsize{9pt}{9pt}\selectfont
  \begin{tabular}{ccc}
  \includegraphics[width=.31\linewidth]{imgs/centerSquare6x6_2a.jpg}
    & \includegraphics[width=.31\linewidth]{imgs/centerSquare6x6_3a.jpg}
    & \includegraphics[width=.31\linewidth]{imgs/centerSquare6x6_4a.jpg} \\
  2 agents & 3 agents & 4 agents
  \end{tabular}
  \subcaption{The lava scenario}
  \label{fig:lava}
\end{minipage}
\begin{minipage}[c]{0.45\linewidth}
  \centering
  \setlength\tabcolsep{1.5pt}
  \fontsize{9pt}{9pt}\selectfont
  \begin{tabular}{cc}
  \includegraphics[width=.45\linewidth]{imgs/appleDoor_a.jpg}
    & \includegraphics[width=.45\linewidth]{imgs/appleDoor_b.jpg}\\
  easy & hard \\  
  \end{tabular}
  \subcaption{The door scenario}
  \label{fig:appledoor}
\end{minipage}
\caption{The discrete gridworld environments. Circles indicate the start locations of the agents, and squares with the same color indicate the corresponding goal locations for each agent.}
\end{figure}

% \begin{figure}[t]
% 	\centering
% 	\subfigure[2 agents]{\includegraphics[width=0.15\textwidth]{imgs/centerSquare6x6_2a.jpg}}
% 	\subfigure[3 agents]{\includegraphics[width=0.15\textwidth]{imgs/centerSquare6x6_3a.jpg}}
% 	\subfigure[4 agents]{\includegraphics[width=0.15\textwidth]{imgs/centerSquare6x6_4a.jpg}}
% 	\caption{The lava scenario. Circles indicate the start locations of the agents, and squares with the same color indicate the corresponding goal locations for each agent.}
% 	\label{fig:lava}
% \end{figure}

% \begin{figure}[t!]
% 	\centering
% 	\subfigure[Easy]{\includegraphics[width=0.22\textwidth]{imgs/appleDoor_a.jpg}}
% 	\hspace{0.02\textwidth}
% 	\subfigure[Hard]{\includegraphics[width=0.22\textwidth]{imgs/appleDoor_b.jpg}}
% 	\caption{The door scenario. Circles indicate the start locations of the agents, and squares with the same color indicate the corresponding goal locations for each agent.}
% 	\label{fig:appledoor}
% \end{figure}





% \begin{figure}[htbp]
%   \centering
%   \subfigure[Agent 1]{\includegraphics[width=0.11\textwidth]{imgs/centerSquare6x6_policy0.jpg}}
%   \subfigure[Agent 2]{\includegraphics[width=0.11\textwidth]{imgs/centerSquare6x6_policy1.jpg}}
%   \subfigure[Agent 3]{\includegraphics[width=0.11\textwidth]{imgs/centerSquare6x6_policy2.jpg}}
%   \subfigure[Agent 4]{\includegraphics[width=0.11\textwidth]{imgs/centerSquare6x6_policy3.jpg}}
%   \caption{Hand-crafted optimal policies for the lava scenario.\yuph{is it necessary to visualize the policy?}}
%   \label{fig:lava-optimal-policy}
% \end{figure}


For each scenario, we collect two sets of demonstrations for each individual agent: optimal and suboptimal. The optimal demonstrations are collected through performing hand-crafted optimal policies in the environments. The suboptimal demonstrations are collected with imperfect policies trained with PPO in the dense-reward setting through an early stopping. We describe the specific rewards in detail later.
%  or trained experts with PPO in the dense-reward setting, where the negative distance between the agent and goal is used as the reward




We compare EG-MARL (Algorithm \ref{algo_EG-MARL}) and GEG-MARL (Algorithm \ref{algo_GEG-MARL}) against four strong baselines: (1) Oracle: the best return one can obtain with optimal policies; (2) MAPPO: training the policies with one of the best decentralized MARL algorithms, MAPPO \citet{yu2021surprising}, in sparse-reward setting; (3) MAGAIL: training the policies with the state-of-art multi-agent imitation learning algorithm, MAGAIL \citet{song2018multi}, under the same setting as ours, where only individual demonstrations are provided; (4) ATA: training the policies with one of the best multi-agent reward-shaping methods, ATA \citet{she2022agent}, in the sparse-reward setting. For each environment, we run each method with 10 different random initializations and plot the mean and variance across all the runs.

% \review{[R3] The colors for the agent and target in the pictures of the policies are a bit confusing since they use the same colors as the agents.}

\paragraph{Task1: The lava scenario} This environment has a 6-by-6 lava pond in the center (see Figure \ref{fig:lava}). We provide three variants of this scenario with varying number of agents and increasing difficulties. The aim of the agents are to reach the corresponding goal locations as soon as possible without stepping into the lava. An episode ends when all agents reach their corresponding goals (succeed), or if any of the agents steps into the lava or the maximum episode length is reached (fail).
The local state space of each agent is its $\{x, y\}$ coordinates in the map. We concatenate all the local states together to form the global state. We assume all agents have access to the global state, which has a dimension of $\mathbb{R}^{n\times2}$ ($n$ is the agent number). The local action space includes five actions: left, right, up, down, and stay. A sparse reward is granted when an episode succeeds, while a small penalty will be subtracted according to the steps taken ($10-\text{step\_count}/\text{max\_step}$). Agents will receive a penalty of $-1$ if they collide with each other.



% \begin{figure}[htbp]
% 	\centering
% 	\subfigure[Agent 1]{\includegraphics[width=0.22\textwidth]{imgs/centerSquare6x6_suboptimal_prior0.jpg}}\hspace{0.02\textwidth}
% 	\subfigure[Agent 2]{\includegraphics[width=0.22\textwidth]{imgs/centerSquare6x6_suboptimal_prior1.jpg}}
% 	\subfigure[Agent 3]{\includegraphics[width=0.22\textwidth]{imgs/centerSquare6x6_suboptimal_prior2.jpg}}\hspace{0.02\textwidth}
% 	\subfigure[Agent 4]{\includegraphics[width=0.22\textwidth]{imgs/centerSquare6x6_suboptimal_prior3.jpg}}
% 	\caption{Agent policies and state occupancy measures estimated from the suboptimal demonstrations for the lava scenario.}
% 	\label{fig:lava-suboptimal-policy}
% \end{figure}

% \begin{figure}[t!]
% \centering
%     \includegraphics[width=0.23\textwidth]{imgs/centerSquare6x6_1a.pdf}
% \caption{An example of personalized demonstrations for the lava scenario (we did not visualize all the optimal paths). There is only one agent in the environment. The agent may take both the left and the right path toward the goal.}
% \label{fig:lava-demon}
% \end{figure}

\begin{table}
\begin{minipage}{0.4\linewidth}
\centering
\includegraphics[width=0.65\textwidth]{imgs/centerSquare6x6_1a.pdf}
\captionof{figure}{An example of personalized demonstrations for the lava scenario (we did not visualize all the optimal paths). There is only one agent in the environment. The agent may take both the left and the right path toward the goal.}
\label{fig:lava-demon}
\end{minipage}\hfill
\begin{minipage}{0.56\linewidth}
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{ccccc}
    \hline
    {{Agent Id}} & {$\mathcal{S}$} & {$\mathcal{A}$} & {Samples} & {Average Episodic Reward} \\ \hline
    1 &  $\mathbb{R}^2$ &  5  & 300  & 4.42  \\ \hline
    2 &  $\mathbb{R}^2$ &  5  & 440  & 4.79  \\ \hline
    3 &  $\mathbb{R}^2$ &  5  & 344  & 4.3   \\ \hline
    4 &  $\mathbb{R}^2$ &  5  & 360  & 4.41  \\ \hline
\end{tabular}}
\caption{The details of suboptimal demonstrations for the lava scenario. The average episodic rewards for optimal demonstrations are around 8.5.}
\label{table:lava-suboptimal-demonstration}
\end{minipage}
\end{table}

% \begin{table}[htbp]
% 	\centering
% 	\resizebox{0.7\columnwidth}{!}{\begin{tabular}{ccccc}
% 		\hline
% 		{{Agent Id}} & {$\mathcal{S}$} & {$\mathcal{A}$} & {Samples} & {Average Episodic Reward} \\ \hline
% 		1 &  $\mathbb{R}^2$ &  5  & 300  & 4.42  \\ \hline
% 		2 &  $\mathbb{R}^2$ &  5  & 440  & 4.79  \\ \hline
% 		3 &  $\mathbb{R}^2$ &  5  & 344  & 4.3   \\ \hline
% 		4 &  $\mathbb{R}^2$ &  5  & 360  & 4.41  \\ \hline
% 	\end{tabular}}
% 	\caption{The details of suboptimal demonstrations for the lava scenario. The average episodic rewards for optimal demonstrations are around 8.5.}
% 	\label{table:lava-suboptimal-demonstration}
% \end{table}

The demonstrations are simply each individual agent moving towards the corresponding goal location, an example is shown in Figure \ref{fig:lava-demon}. Note that the personalized demonstrations do not specify which direction the agents should take to avoid colliding with the others. When training suboptimal PPO policies, we define the dense reward as the negative distance between the agent and the goal, and the episode terminates once the agent reaches the goal or steps into lava. 
% We visualize the optimal and suboptimal policies in Figure \ref{fig:lava-optimal-policy} and \ref{fig:lava-suboptimal-policy} respectively. The red square represents the start position of the agent, and the green square represents its corresponding goal location. The arrows represent the actions that can be taken at each state, and the length of each arrow represents the probability of that action. 
The details of the suboptimal demonstrations are summarized in Table \ref{table:lava-suboptimal-demonstration}. The average episodic rewards for optimal personalized demonstrations are about twice of the suboptimal ones.



% \review{[R1] The impact of the batch size is analyzed (text and Fig 5) but does not correspond to the 4 points mentioned initially in the Experimental evaluation. Further, since there is no apparent impact in the range explored, I would suggest removing that.}

% \review{[R3] It is not clear which policy was used to generate the demonstrations in Fig 5.}

% % \textbf{Evaluation of the batch size for occupancy measure estimation.} 
% We first explore the impact of the batch size $B$ for empirical occupancy measure estimation in Algorithm \ref{algo_2}. We compare among $B = \{100, 1000, 10000\}$. It was originally expected that the learned policy would converge faster and reaches higher returns with a larger batch size since the occupancy measure estimation would be more accurate. However, it turns out to be not such case as we observe from the experiment results shown in Figure \ref{fig:lava-ns}. It can be seen that all the learning curves converge at a similar rate with different values of $B$.

% \begin{figure}[b!]
% 	\begin{center}
% 		\includegraphics[width=0.6\linewidth]{imgs/lava_2a_Ns.pdf}
% 	\end{center}
% 	\caption{lava (2-agent case) environment with varying numbers of samples for computing the occupancy measure. \yuph{remove this figure, the results hurt our story. But it's an interesting question to ask: How many samples are enough to obtain a good occupancy measure estimation?(check Hoeffding's inequality.) How good an occupancy measure should be to get a good training result?}}
% 	\label{fig:lava-ns}
% \end{figure}



% \review{[R2] In fig. 6, could authors explain why sometimes policies trained by suboptimal demonstrations achieved better performance than policies trained by optimal demonstrations? And why do policies trained by optimal demonstrations show much higher variances compared to policies trained by suboptimal demonstrations?}


% Behavior: shall we use a sub-optimal policy? (Train the environment with a dense reward using ppo and stops early to obtain a sub-optimal policy)

\paragraph{Task 2: The door scenario} This environment is adapted from \citet{franzmeyer2022learning} (see Figure \ref{fig:appledoor}). The green agent needs to step onto the green square and stay there to keep the door open and let the red agent enter the right room. An episode ends when the red agent reaches the red goal location (succeed), or the maximum episode length is reached (fail). The state and action space are the same as the lava environment. The reward is also defined similarly: a sparse reward is granted when the agent reaches the red goal based on the total steps taken, and agents will receive a penalty of $-1$ if they collide with each other.
% whose value is calculated according to the steps taken ($10-\text{step\_count}/\text{max\_step}$)

% \begin{figure}[htbp]
% 	\centering
% 	\subfigure[Case a, Agent 1]{\includegraphics[width=0.22\textwidth]{imgs/appleDoor_a_prior0.jpg}}\hspace{0.02\textwidth}
% 	\subfigure[Case a, Agent 2]{\includegraphics[width=0.22\textwidth]{imgs/appleDoor_a_prior1.jpg}}
% 	\subfigure[Case b, Agent 1]{\includegraphics[width=0.22\textwidth]{imgs/appleDoor_b_prior0.jpg}}\hspace{0.02\textwidth}
% 	\subfigure[Case b, Agent 2]{\includegraphics[width=0.22\textwidth]{imgs/appleDoor_b_prior1.jpg}}
% 	\caption{Agent policies and state occupancy measures estimated from the optimal demonstrations for the door scenario.}
% 	\label{fig:appledoor-optimal-demonstration}
% \end{figure}


The demonstrations are the red agent moving toward the red square with the door open, and the green agent moving toward the green square. The dense reward is defined similarly when we train suboptimal PPO policies, and each episode terminates once the agent reaches the goal. 
% We visualize the optimal and suboptimal policies and the estimated occupancy measures in Figure \ref{fig:appledoor-optimal-demonstration} and \ref{fig:appledoor-suboptimal-demonstration} respectively. The representations are the same as the lava scenario. 
The details of the suboptimal demonstrations are summarized in Table \ref{table:appledoor-suboptimal-demonstration}. The average episodic rewards for optimal personalized demonstrations are about twice of the suboptimal ones as well.




\begin{table}[htbp]
\centering
\resizebox{0.65\columnwidth}{!}{\begin{tabular}{c|ccccc}
\hline
\textbf{Case}  & \textbf{Agent} & \textbf{$\mathcal{S}$} & \textbf{$\mathcal{A}$} & \textbf{Samples} & \textbf{Average Episodic Reward} \\ \hline
\multirow{2}{*}{easy} & red    & $\mathbb{R}^2$    & 5   & 643   & 4.01   \\ \cline{2-6} 
                   & green    & $\mathbb{R}^2$    & 5   & 612   & 4.39   \\ \hline
\multirow{2}{*}{hard} & red    & $\mathbb{R}^2$    & 5   & 607   & 4.34   \\ \cline{2-6} 
                   & green    & $\mathbb{R}^2$    & 5   & 593   & 4.36   \\ \hline
\end{tabular}}
	\caption{The detail of suboptimal demonstrations for the door scenario. The average episodic rewards for optimal demonstrations are around 9.}
	\label{table:appledoor-suboptimal-demonstration}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%% exp results
\textbf{Results. }
We compare EG-MARL and GEG-MARL with other baseline methods on both the lava and the door scenarios using optimal and suboptimal demonstrations. In the lava scenario, we demonstrate the scalability of our algorithms to a varying number of agents, while in the door scenario, we show the effectiveness of our algorithm in a heterogeneous setting.



\begin{figure*}[t]
\centering
\begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[width=0.78\textwidth]{imgs/lava_optimal.pdf}
    \caption{Experiments with optimal demonstrations}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[width=0.78\textwidth]{imgs/lava_suboptimal.pdf}
    \caption{Experiments with suboptimal demonstrations}
\end{subfigure}
\caption{Learning curves of our algorithms versus other baseline methods under the lava scenario. The proposed EG-MARL and GEG-MARL algorithms converge to higher rewards compared to the baseline models. It also can be seen that GEG-MARL generalizes better to larger numbers of agents.}
\label{fig:lava-exp-results}
\end{figure*}



The learning curves in the lave scenario are shown in Figure \ref{fig:lava-exp-results}, which demonstrate that EG-MARL performs the best in the 2-agent case, but converges much slower in 3-agent and 4-agent cases. GEG-MARL shows much better generalizability to a larger number of agents --- it can explore efficiently in all three settings and performs stably even with suboptimal demonstrations. MAPPO fails to learn any meaningful behavior in all cases due to the reward being too sparse. MAGAIL performs even worse than MAPPO: the agents keep colliding with each other using the learned policy. This is not surprising since MAGAIL does not have access to the environmental reward signal and simply imitates the individual agent demonstrations, thus cannot obtain any feedback when collaborations are necessary. ATA can learn suboptimal policies for the 2-agent case, but fails to learn as the agent number grows. 


Figure \ref{fig:appledoor-exp-results} shows the learning curve comparison between our algorithms and other baseline methods in the door scenario. The easy case is more straightforward: the green agent must navigate to the green square and stay there to keep the door open, thus allowing the red agent to enter the right room and navigate to its goal location. Almost all the algorithms but MAGAIL perform well in this case, among which EG-MARL converges the fastest. Intuitively, simply following individual demonstrations should lead to success. MAGAIL fails because the green agent does not learn to stay at the green square by imitating the demonstrations -- the demonstrations do not involve the desired action when the agent is on the green square. This further emphasizes the importance of environmental reward signals if individual demonstrations are adopted for multi-agent learning. The hard case is much more complex and requires more agent collaboration. The green agent must first open the door and stay there to let the red agent enter the middle room, then move away from the green square to allow the red agent to enter the right room and navigate toward the goal location. Only GEG-MARL converges well under such a setting. The discriminator provides more variability in reward change and brings about better convergence.

% Figure \ref{fig:appledoor-exp-results} presents a comparative analysis of the learning curves for our algorithms and baseline methods within the door scenario. In the straightforward instance, the task entails the green agent reaching the green square and maintaining its position to facilitate the passage of the red agent into the adjacent room, thereby enabling the latter to progress towards its designated goal location. Most algorithms, with the exception of MAGAIL, demonstrate proficient performance in this context. Notably, EG-MARL exhibits the swiftest convergence, as it intuitively aligns with the successful outcome of adhering to individual demonstrations. It is imperative to highlight that MAGAIL falls short in this scenario due to its inability to instruct the green agent to remain stationed at the green square as the demonstrated behaviors do not encompass the requisite action when the agent occupies said square. This underscores the critical significance of environmental reward signals when integrating individual demonstrations into multi-agent learning paradigms.

% Conversely, the more intricate scenario necessitates a higher degree of agent cooperation. Here, the green agent must initially open the door and maintain its position to allow the red agent access to the middle room. Subsequently, the green agent must disengage from the green square, thereby permitting the red agent to proceed into the right room and navigate towards its ultimate goal. In this complex setting, only GEG-MARL demonstrates commendable convergence. This can be attributed to the discriminator introducing increased variability in reward alterations, thereby fostering superior convergence dynamics.

% \begin{table}
% \centering
% \resizebox{0.65\columnwidth}{!}{\begin{tabular}{c|ccccc}
% \hline
% \textbf{Case}  & \textbf{\begin{tabular}[c]{@{}c@{}}Agent\\ Id\end{tabular}} & \textbf{$\mathcal{S}$} & \textbf{$\mathcal{A}$} & \textbf{Samples} & \textbf{\begin{tabular}[c]{@{}c@{}}Average \\ Episodic Reward\end{tabular}} \\ \hline
% \multirow{2}{*}{a} & 1    & $\mathbb{R}^2$    & 5   & 643   & 4.01   \\ \cline{2-6} 
%                   & 2    & $\mathbb{R}^2$    & 5   & 612   & 4.39   \\ \hline
% \multirow{2}{*}{b} & 1    & $\mathbb{R}^2$    & 5   & 607   & 4.34   \\ \cline{2-6} 
%                   & 2    & $\mathbb{R}^2$    & 5   & 593   & 4.36   \\ \hline
% \end{tabular}}
% 	\caption{The detail of suboptimal demonstrations for the door scenario.}
% 	\label{table:appledoor-suboptimal-demonstration}
% \end{table}

% \review{[R3] Consider renaming the labels in Figure 8 to Agent red and agent green}
% \begin{figure}[htbp]
% 	\centering
% 	\subfigure[Case a, Agent 1]{\includegraphics[width=0.22\textwidth]{imgs/appleDoor_a_suboptimal_prior0.jpg}}\hspace{0.02\textwidth}
% 	\subfigure[Case a, Agent 2]{\includegraphics[width=0.22\textwidth]{imgs/appleDoor_a_suboptimal_prior1.jpg}}
% 	\subfigure[Case b, Agent 1]{\includegraphics[width=0.22\textwidth]{imgs/appleDoor_b_suboptimal_prior0.jpg}}\hspace{0.02\textwidth}
% 	\subfigure[Case b, Agent 2]{\includegraphics[width=0.22\textwidth]{imgs/appleDoor_b_suboptimal_prior1.jpg}}
% 	\caption{Agent policies and state occupancy measures estimated from the suboptimal demonstrations for the door scenario.}
% 	\label{fig:appledoor-suboptimal-demonstration}
% \end{figure}




\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.49\textwidth}
     \centering
     \includegraphics[width=\textwidth]{imgs/appleDoor_optimal.pdf}
     \caption{Experiments with optimal demonstrations}
     % \label{}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
     \centering
     \includegraphics[width=\textwidth]{imgs/appleDoor_suboptimal.pdf}
     \caption{Experiments with suboptimal demonstrations}
     % \label{}
\end{subfigure}
% \subfigure[Experiments with optimal demonstrations]{\includegraphics[width=0.49\textwidth]{imgs/appleDoor_optimal.pdf}}
% \subfigure[Experiments with suboptimal demonstrations ]{\includegraphics[width=0.49\textwidth]{imgs/appleDoor_suboptimal.pdf}}
\caption{Learning curves of our algorithms versus other baseline methods under the door scenario. Our proposed GEG-MARL algorithm demonstrates better robustness in terms of convergence and generalizability.}
\label{fig:appledoor-exp-results}
\end{figure}



\subsection{The continuous Multi-Agent Particle environment}

We modified the cooperative navigation task of multi-agent particle environment~\citet{lowe2017multi, mordatch2017emergence} to evaluate the performance of our algorithm in a continuous environment. 
%
We only compare GEG-MARL versus MAPPO on this task. EG-MARL cannot be used for this task since it is not feasible to estimate occupancy measures through Monte Carlo rollouts in the continuous setting. We do not compare with MAGAIL, since, as the discrete environments show, simply imitating the experts is not sufficient.

\begin{figure}[t]
\centering
\begin{subfigure}[c]{0.25\columnwidth}
     \includegraphics[width=\textwidth]{imgs/mpe.png}
     \caption{}
\end{subfigure}
\hspace{0.05\columnwidth}
\begin{subfigure}[c]{0.35\columnwidth}
     \includegraphics[width=\textwidth]{imgs/mpe.pdf}
     \caption{}
\end{subfigure}
% \subfigure[]{\includegraphics[width=0.3\columnwidth]{imgs/mpe.png}}
% \subfigure[]{\includegraphics[width=0.45\columnwidth]{imgs/mpe.pdf}}
\caption{(a) The modified cooperative navigation scenario. (b) Learning curves of GEG-MARL versus MAPPO under the modified cooperative navigation scenario.}
\label{fig:mpe_res}
\end{figure}

% \begin{figure}[h]
% 	\begin{center}
% 		\includegraphics[width=0.65\linewidth]{imgs/mpe_res.pdf}
% 	\end{center}
% 	\caption{Learning curves of GEG-MARL versus MAPPO under the modified cooperative navigation scenario.}
% 	\label{fig:mpe_res}
% \end{figure}


\paragraph{Cooperative Navigation}
The modified environment consists of 2 agents, 2 goal landmarks, and 1 wall between the agents and the goals. The agents need to navigate around the wall to occupy both landmarks. The state definition is the same as the original. We sparsify their original reward as follows:
\begin{equation}
    r = \sum_{a \in A} \min (0.3, \min_{g \in G} d(a, g)) + \sum_{g \in G} \min(0.3, \min_{a \in A} d(a, g)). 
\end{equation}
%
Figure \ref{fig:mpe_res} demonstrates the learning curves of both algorithms. This validates the ability of GEG-MARL in continuous environments.





%\subsection{The StarCraft environment}



